The End of Slow Networks: It's Time for a Redesign

Next generation high-performance RDMA-capable networks will require a fundamental rethinking of the design and architecture of modern distributed DBMSs. These systems are commonly designed and optimized under the assumption that the network is the bottleneck: the network is slow and "thin", and thus needs to be avoided as much as possible. Yet this assumption no longer holds true. With InfiniBand FDR 4x, the bandwidth available to transfer data across network is in the same ballpark as the bandwidth of one memory channel, and it increases even further with the most recent EDR standard. Moreover, with the increasing advances of RDMA, the latency improves similarly fast. In this paper, we first argue that the "old" distributed database design is not capable of taking full advantage of the network. Second, we propose architectural redesigns for OLTP, OLAP and advanced analytical frameworks to take better advantage of the improved bandwidth, latency and RDMA capabilities. Finally, for each of the workload categories, we show that remarkable performance improvements can be achieved.

==> ml.tex <==
\section{Advanced Analytics}
\label{sec:ml}

The previous sections showed that distributed database system for OLTP and OLAP have to be redesigned to take full advantage of the next generation of networks. 
In this last section, we argue that recent in-memory analytics frameworks (e.g., Spark~\cite{spark}, Tupleware~\cite{crotty2014tupleware}) must also change to leverage high-performance networks.
Machine learning (ML) tasks are a popular use-case for these frameworks, but existing algorithms and systems make the wrong assumptions about the network.

\textbf{Background:}
Many ML algorithms can be distributed using a very simple pattern~\cite{mahout}: first, the training data is randomly partitioned across worker nodes in a cluster, and a randomly initialized model is replicated on every node.
Each worker optimizes its local state using a loss function on its local data before sending delta updates of the model to the master node. 
The master combines all delta updates to produce a new global state, which is then redistributed to all nodes.
For example, an implementation of logistic regression using batch gradient descent would iteratively refine a weight vector by applying the incremental updates computed by each worker. 
While many algorithms have small models (e.g., logistic regression only requires one weight value for each relevant attribute), others can have large shared state (e.g., PageRank).
Especially with slow Ethernet networks, the redistribution of large models between every iteration often becomes the bottleneck.

Unsurprisingly, many algorithms have been proposed to avoid replicating the full state across all the machines (e.g., \cite{andrewng,commavoidingml}).
Yet again, these algorithms are based on the now-incorrect assumption that the network is the bottleneck, and we argue that they will require substantial redesigns in order to take full advantage of new network technologies.

Since the bandwidth of InfiniBand is similar to the bandwidth of the memory bus, it is no longer the best strategy to avoid communication at all costs. 
To prove this point, we compared two PageRank implementations that use a relation to represent the sparse adjacency matrix: (1) a textbook version of the algorithm \cite{manning2008introduction}, and (2) a communication-avoiding version~\cite{pagerankp2p} that sends only updated (i.e., non-converged) ranks on each iteration.
The core idea is that the ranks of many pages (e.g., those with no inbound links) converge after only a few iterations, and it is therefore unnecessary to continually redistribute these weights on subsequent iterations.
This communication-avoiding optimization is similar to the semi-join algorithm described in Section~\ref{sec:olap:bloom} that spends extra CPU time to minimize the number of tuples sent over the network.

\textbf{Evaluation:}
We tested both algorithms with 1M pages (20GB of data) on 4 servers using 40 iterations with the same system and network configuration described in the previous section.
As Figure~\ref{fig:ml} shows, the communication-avoiding algorithm outperforms the classic implementation on a traditional network.
However, the classic version is more efficient using IPoIB because the communication-avoiding algorithm spends substantially more CPU time trying to save network bandwidth, which is no longer a scarce resource.
Of course, the speedup depends on the data and details of the implementation.
Also we do not argue, that with the next generation of networks avoiding communication is necessarily a bad thing. 
However, these results suggest that the bottleneck is shifting away from the network and that a stronger focus should be placed on CPU efficiency, as some recent projects have started to explore~\cite{crotty2014tupleware}.

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{experiments/ml.pdf}
\vspace{-12pt}
\caption{Classic vs. Comm.-Avoiding PageRank}
\vspace{-15pt}
\label{fig:ml}
\end{figure}

%
%  TO DO (TIM)
%
%Future (Tim)
%distributed hogwild
%new algorithms
%clever systems optimizations (e.g., better use caches and rdma to update state on remote machines -> graphlab)
%
%Overview
%- many ML algorithms have very large shared state and are hard to partition (e.g., pagerank, neural networks).
%- the conventional wisdom is to avoid communication whenever possible in order to improve performance
%- avoiding communication is done at the cost of increased CPU time
% - we argue that algorithms must change in order to optimally utilize fast networks.
%
%- Pagerank
%- BS overview (iterative, popular web algorithm...)
%- two ways of implementing it
%
%1) Simplest (non-communication avoiding)
%- partition links input across n workers
%- on each iteration, master receives an update (delta) to the rank values for each page in the data set
%- once master has received updates for each page (from each of the n workers), apply the "teleportation" formula and redistribute the rank values to each worker.
%- Total data transfer (assuming floats):
%#iterations * #workers * #pages * 4 bytes
%- the form of the ranks that are being sent (from each worker to the master) a 1-d float array (where the page# is an offset into the array)
%- when updates from each worker are merged, the access pattern is sequential (merging two arrays).  Nice cache utilization/prefetching. 
%
%2) Optimization (communication avoiding)
%- Instead of having each worker send updates for each page, only send updates that are > some threshold (epsilon).
%- Idea is that the rank values for many pages converge quickly (e.g., pages that have no inbound links will be 0).
%- The amount of data sent over the network decreases as more and more pages converge (cite [1])
%- Total data transfer (assuming floats)
%#iterations * #workers * k * #pages * 8 bytes
% where 0 <= k <= 1 and gets smaller on every iteration (8 bytes bc key,value pairs)
% - since the updates are sparse, each worker needs to send a set of (page,delta) pairs to the master (instead of an array).
% - poor cache performance when merging updates on the master (random access)
% - need to send 2x more data when k = 1
%
%3) Evaluation
%- compare the simple algorithm with the communication avoiding algorithm
%for slow networks, communication avoiding algorithm is faster, while for fast networks the simple algorithm is faster.
% results: https://docs.google.com/a/brown.edu/spreadsheets/d/1RMJeGlz3khq8YbvtQa6DujlVWNamppq5dzUgzOu2k0o/edit#gid=0
% [1] - http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.13.9589

==> response.tex <==
\begin{appendices}
\section{Response for Paper \#498}
\noindent Dear VLDB Associate Editor and Reviewers:

We would like to thank you for the very helpful feedback on our paper.
We have addressed all listed concerns and included references to the revised text below.
As requested by the Associate Editor, we focused especially on the detailed comments of Reviewer 2, but we also addressed the comments of the other reviewers.
To summarize:
\begin{packed_item}
  \item We added an experiment to demonstrate that the network bandwidth can indeed saturate the main memory bandwidth rather than relying solely on published specifications.
  \item We updated all RDMA OLTP benchmarks with our latest implementation and a larger cluster setup, achieving a higher throughput and better scalability.
  \item We extended the OLAP section to discuss and evaluate and additional common operator, including new experiments.
  \item We extended the related work section to discuss the suggested literature and systems.
\end{packed_item}

\subsection{Reviewer 2}
\textit{\textbf{W1: One base point the paper raises is that RDMA is faster than main memory in bandwidth and is in a similar range of latency (0.1us versus 0.08us respectively in their experiments). However, there is no experiment in the paper comparing these two in the paper's experimental setup. Figure 1 seems to draw bandwidth numbers from existing studies [1] and [7].}}

\textit{\textbf{D1: My main complaint is that, even though the paper claims that RDMA is comparable with local memory latency and even faster in bandwidth, the experiments did not show this point sufficiently.}}

We added a new experiment to the introduction (Figure~\ref{fig:bandwidth_mem_ib}) showing that the network can indeed match the memory bandwidth.
In this experiment, we reconfigured our cluster to use 2 NICs per socket (i.e., 4 NICs per node).
The detailed hardware description and setup of the experiment can be found in the introduction.

According to the specification, our machines should have an available memory bandwidth of 102 GB/s, whereas we only measured 78.4 GB/s.
For measuring the memory bandwidth, we used the parallel memory bandwidth \emph{pmbw}\footnote{\url{https://panthema.net/2013/pmbw/}} which achieved a maximum bandwidth of $74$ GB/s.
Moreover, in order to verify the bandwidth, we implemented our own memory benchmark\footnote{ \url{https://github.com/BrownBigData/numabench}} which allows us to allocate memory on a given NUMA region and pin threads to the corresponding cores.
With our benchmark, we achieved the previously mentioned $78.4$ GB/s.
We measured the bandwidth of the InfiniBand network using the official \emph{perftest} package provided by the OFED driver installation from Mellanox.

Since these measurements represent a rather large difference from the theoretical bandwidth, we compared our results to other memory bandwidth benchmarks, which report similar numbers (e.g., see the large array parallel results of the 2 socket E5 machines of \url{https://panthema.net/2013/pmbw/results.html}).
Therefore, we speculate that the network bandwidth can match not only the memory bandwidth of the DDR3-1600 memory in our cluster, but should also be able to match the memory bandwidth of DDR3 RAM with much higher data rates (e.g., DDR3-2133), since the Infiniband NICs can achieve transfer rates much closer to the specification (based on our microbenchmark). 

We believe that this experiment shows that the network bandwidth can fully saturate the available memory bandwidth.
In addition, we also clarified the text according to the reviewer's suggestion.
Finally, both the memory and network latency measurements referenced in the introduction ($0.1\mu s$ vs $0.08\mu s$) were measured on the same hardware and are not based on the specification.

\textit{\textbf{W2. The paper proposes the NAM architecture in which the database system treats the aggregated RAM across nodes as a distributed memory pool. This setup is desirable to the database application programs; however, the management of such a storage system, especially for OLTP workloads, would be complex and the scalability a major concern.}}

We agree that this design might add some complexity for global memory management.
However, it also provides significant benefits regarding scalability, as shown in our OLTP benchmarks.
Moreover, we also believe that a NAM architecture can remove some of the complexities associated with a distributed DBMS.
For example, many shared-nothing systems use two transaction protocols, one locally within a partition and another one for cross-partition transactions. 
In contrast, our NAM design requires only a single transaction protocol for the entire system, thereby simplifying the design. 
Similar complexities can be removed for distributed OLAP queries (e.g., avoiding adding additional data reduction techniques like semi-joins).

Regardless of these arguments, as a vision paper, we want to outline the benefits of this approach and hope that it will create a fruitful new area of research to address the various problems, including design complexity and scalability. 

\textit{\textbf{D2) The "rethinking the architecture" section presents both the shared memory over RDMA option and the NAM (RDMA) proposal. In essence, the divide is in whether the shared memory communication is implemented in the OS (SM over RDMA) or in the DBMS (NAM). The paper advocates NAM; however, there is little experimental comparison on SM over RDMA in the paper. Especially, it claims that the SM over RDMA option is entirely omitted in OLAP comparison that this option is similar to Shared-Nothing with IPoIB architecture. I wonder how the author could fix this absence of SM over RDMA without totally dismissing an interesting option.}}

We reached out to IBM to get access to their SM implementation over RDMA.
Unfortunately, their software is incompatible with our hardware, and it is still unclear if we would be allowed to share any performance results.
Similarly, implementing our own real SM RDMA solution from scratch would take a prohibitively long amount of time.
Without having access to existing software, it is very hard to precisely quantify the difference, but we hope that we can tackle this problem in the future ourselves (e.g., by getting access to IBM's infrastructure) or that other researchers will be inspired by this vision paper to perform such an analysis themselves.

In addition, we would like to point out that we do evaluate a hand-coded SM architecture with \texttt{send/receive} in the OLTP section (though, arguably, it is not exactly the same).
This implementation performs significantly worse than our RSI implementation with NAM (the new experiments and descriptions are included in the revision).

We omitted a hand-coded SM architecture entirely for our OLAP comparison, since two-sided RDMA verbs would have added synchronization overhead to our system (i.e., an RDMA RECEIVE must be issued strictly before the RDMA SEND arrives at the NIC), which would have greatly slowed down the execution of our OLAP algorithms.

Finally, we argue that since virtual memory was never a particularly useful abstraction for DBMSs, the usefulness of distributed shared memory for distributed DBMSs is similarly suspect, even with RDMA.
Admittedly, these are only anecdotal arguments, and we yet again hope that our vision paper inspires additional research in this area.

\textit{\textbf{W3. The proposal of RSI is sketchy, and the experiments compared only up to 40 clients (threads) executing on 10,000 products on four servers. As such, it sounds a bit unconvincing to conclude that distributed transactions no longer have a scalability concern and that partitioning schemes might be unnecessary in many scenarios.}}

Just to clarify, in the original submission, our experiment used six servers (four acting as NAM-servers and two as ``client'' application servers).
The client machine is in fact a server since it actually implements the transaction protocol.

For the resubmission, we changed the entire experiment to better show the scalability.
Now the experiment runs on eight servers: one acting as a timestamp server, three as NAM storage servers, and four as clients (i.e., compute servers).
Moreover, we implemented a new wait-free timestamp technique, removing it as the main bottleneck in the system.
Because of the change, our current RSI implementation is able to handle up to $\approx 1.8M$ distributed transactions per second with 70 clients.
With more than 70 clients, the network bandwidth gets fully saturated, since our default cluster configuration has only one dual-port FDR 4x NIC per machine (not four as required to match the main memory bandwidth).
We therefore updated the OLTP section to include the new results and also added a theoretical discussion of the throughput limit.
In addition, we removed the transaction latency experiment as it no longer adds much value.

Based on these new results, we still speculate that the RSI protocol will continue to scale.
However, since we also do not know for certain, we softened the language in the text to make it clearer that we are speculating.
Since this is a vision paper, we believe such speculations are actually encouraged and add value to the overall argument.

\textit{\textbf{D3. I understand that a vision paper can make big claims with small cases. Nevertheless, it sounds a bit overreaching to represent OLAP with a join algorithm.}}

In our case for OLAP, we added a subsection and an experimental evaluation for the second most common OLAP operation: aggregation.
The experiment shows the exact same behavior as the join; with a fast network, the bottlenecks are shifting, and cache-efficiency and fine-grained parallelism are more important than minimizing network communication.
In addition, we made it clearer in the text (at the end of experimental section) that we use our results to speculate how the network will change the DBMS architecture for the OLAP world.

\textit{\textbf{D4. The paper has quite a few back-of-envelop calculations, and plots the per-message CPU overhead in CPU cycles with respective to message size. I understand the network throughput and latency measurement, and wonder how the CPU overhead is measured or calculated. Does the CPU overhead including local memory access? Is there overlap between CPU overhead, local memory access, and network communication?}}

For measuring the CPU overhead, we used an end-to-end experiment that includes the full stack (from local memory access to network communication).
In order to deal with asynchronous execution in the OS, we used a ping/pong experiment that sends a message from the client to the server and back.
In order to include all costs of the complete stack, we read the cycle counter of our CPU using the RDTSC instruction before sending the ping and after receiving the pong.
The RDTSC instruction reads a register of Intel CPUs that represents a timestamp counter to keep track of every cycle that occurs on a CPU.
The cycles that we have plotted in our paper for a given message of size $x$ represent half the cycles needed for the full round-trip of $x$.

\textit{\textbf{D5. The overhead of multiple versions of data items is usually considered in snapshot isolation. Is it relevant in a cluster environment, especially in the proposed NAM architecture?}}

It is correct that keeping track of multiple versions is not ``for free.''
However, there are several ways to deal with it.
On one hand, we could (per default) only read the latest version (as done in our experiments) and only if needed, fetch an older version.
Since it is reasonable to assume that most transactions require the latest version, this protocol only adds additional latency for a few transactions.
In cases where the network bandwidth matches the main memory bandwidth, the only difference from an in-memory DBMS is that the latency to fetch an older version is higher.

In contrast, if we always fetch the current and several older versions (as described in the paper) to reduce the latency, we might saturate the network/memory bandwidth earlier.
So yes, multiple versions can have an impact in the cluster environment. 

We believe that we have just started to understand these trade-offs and that there are many interesting ways to mitigate the impact of multiple versions (e.g., leveraging two-sided verbs, RDMA NICs with FPGA features).
Also, there are many different ways to implement multiple versions and perform the bookkeeping.
Again, in the spirit of the vision paper, we extended the description of these challenges to encourage more research in the future in these areas.

\subsection{Reviewer 1}
\textit{\textbf{W1. The paper does not provide sufficient evidence that advances in RDMA-capable networking requires a fundamental rethinking of in-memory DBMSes. The case for 2PC-bound workloads is clear. This claim could be strengthened with data arguing how many in-memory OLTP workloads are currently 2PC bound. Do we expect this to be an increasingly important problem in the future?}}

Given that even weakly-consistent NoSQL systems are steadily moving towards stronger consistency guarantees (e.g., Google's F1 system uses 2PC), we believe that strong consistency will remain an important problem in the future.
As argued in the paper, not every workload is easily partitionable, and thus, there will always be a need for distributed coordination.
Even more importantly, many current techniques (e.g., workload partitioning, load partitioning) might become obsolete with modern RDMA-capable networks and our proposed designs.
These architectures could significantly simplify the design of distributed DBMSs.
We tried to make some of these arguments clearer in the text.

\textit{\textbf{2. The application to OLAP is a rather weak part of the paper. In particular, the novelty, and improvements wrt [11] are fairly incremental. I'm not convinced that the IB networking stack produces the same order of improvements from re-architecting a main-memory OLAP workloads as it does for 2PC-bound OLTP workloads.}}

While it is true that the difference between our join algorithm and [11] are rather minor (we developed our algorithm in parallel to [11]), the important takeaway of the OLAP case is that the techniques of the current distributed DBMSs have to change.
For example, communication-avoiding algorithms (e.g., semi-joins) are no longer beneficial. 
We therefore provide a more theoretical analysis of join algorithms, which we believe are important and ignored by [11].

In addition, we also strengthened the OLAP section and now include experiments for an aggregate operator (see also the answer for comment D2 of Reviewer 2).

\textit{\textbf{3. IIRC, RDMA atomic operations are used in Oracle RAC in the lock manager (and perhaps other designs like IBM DB2 purescale). Commercial DBMSes have made limited use of RDMA for several years. At the very least, you should discuss this in related work beyond just saying that they were designed when bandwidths were lower.}}

Thank you for the suggestions and pointing towards the products.
We expanded the related work section to include the mentioned systems.

\subsection{Reviewer 3}
\textit{\textbf{1. My main disagreement with the paper’s direction is the lack of attention to the software overhead in architecting around antiquated technologies---history shows that the biggest benefits come when an entire design philosophy changes and not when we optimize around the speed improvement of new technologies. For example, instead of focusing on reducing software overhead the paper proposes more complex storage access operations. History has also shown that specialized hardware (such as the paper’s RNIC proposal) doesn’t win over commodity CPUs (see original database machine, followed by Netezza’s move away from FPGAs, and most recently the lack of traction of GPUs).}}

While we agree with the reviewer that in the past this observation was indeed true, it is still unclear if it will remain true in the future.
However, we believe that the next generation of networks actually also provides an opportunity to reduce the software overhead.
While the storage operations might be more complex, many of the algorithms can be simplified due to the faster network.
For example, RDMA-optimized radix joins are much simpler than radix joins that use semi-reductions.
Similarly, many of the complex data partitioning and load-balancing techniques become obsolete and can be replaced by much simpler solutions.
New network properties also encourage a redesign of the way we achieve durability and what types of redo-logs we really need, again potentially simplifying the architecture.
We have updated the text to better emphasize this excellent point.

\textit{\textbf{2. Rethinking “traditional” in-memory distributed DBs: not so traditional, haven’t caught on yet.}}

Thank you for pointing this out.
We are now more careful with the word ``traditional.''

\textit{\textbf{4. “Cost-based optimizers have to change”: I’d be more careful here. Especially for in-memory DBMSs where optimizers don’t play a big role.}}

While arguably cost-based optimizers play only a small role for in-memory DBMSs on a \textit{single} node, they do play a very important role for distributed DBMSs.
As argued in Section 3.2, current cost-based models for distributed systems try to avoid communication.
Therefore, they have to change for RDMA.

To avoid this confusion (distributed vs in-memory cost-based optimizers), we clarified the text accordingly. 

\textit{\textbf{5. NAM is interesting. Simple and at the same time powerful.}}

Thank you!

\textit{\textbf{6. Minor comments: Figure 4(b): how is it different than (a) ?}}

They are indeed very similar.
We just wanted to visualize the Ethernet case rather than ignoring it.

\textit{\textbf{Decoupled compute/storage: need to mention Microsoft SQL Azure DW, Snowflake.}}

Thank you for pointing these out.
We have updated the text to reference these systems.

\textit{\textbf{Section 3.2: “prefetching using selective signaling” please elaborate.}}

We have added a sentence to explain the idea of prefetching in Section 3.2 better.
\end{appendices}
